EVOLIN Benchmark: Evaluation of Line Detection and Association

Lines are interesting geometrical features commonly seen in indoor and urban environments. There is missing a complete benchmark where one can evaluate lines from a sequential stream of images in all its stages: Line detection, Line Association and Pose error. To do so, we present a complete and exhaustive benchmark for visual lines in a SLAM front-end, both for RGB and RGBD, by providing a plethora of complementary metrics. We have also labelled data from well-known SLAM datasets in order to have all in one poses and accurately annotated lines. In particular, we have evaluated 17 line detection algorithms, 5 line associations methods and the resultant pose error for aligning a pair of frames with several combinations of detector-association. We have packaged all methods and evaluations metrics and made them publicly available on web-page https://prime-slam.github.io/evolin/.

==> tables/association_fps.tex <==
\begin{table}[!htb]
\centering
\caption{Association performance}
\label{table:association_fps}
\resizebox{1\linewidth}{!}{
\begin{tabular}{|l||l|l|l|l|} 
\hline
\multirow{2}{*}{Algorithm} & \multicolumn{4}{c|}{FPS}                                 \\ 
\cline{2-5}
                           & lr kt2      & of kt2      & fr1/desk     & fr3/cabinet   \\ 
\hline
{LBD}               & \textbf{94} & \textbf{80} & \textbf{109} & \textbf{195}  \\
{DLD}               & \uline{31}  & \uline{16}  & \uline{23}   & \uline{74}    \\
{WLD}               & 4           & 2           & 3            & 13            \\
{LineTR}            & 14          & 12          & 14           & 19            \\
{SOLD2}             & 2           & 1           & 2            & 4             \\
\hline
\end{tabular}
}
\end{table}

==> tables/detection_fps.tex <==
\begin{table}[!htb]
\centering
\caption{Detection performance}
\label{table:detection_fps}
\resizebox{0.65\linewidth}{!}{
\begin{tabular}{|l||l|l|l|l|} 
\hline
\multirow{2}{*}{Algorithm} & \multicolumn{4}{c|}{FPS}                                   \\ 
\cline{2-5}
                           & lr kt2       & of kt2       & fr1/desk     & fr3/cabinet   \\ 
\hline
AFM                        & 12           & 12           & 11           & 10            \\
ELSED                      & 107          & 98           & 69           & 162           \\
F-Clip                     & 30           & 29           & 29           & 29            \\
HAWP                       & 25           & 23           & 23           & 26            \\
HT-LCNN                    & 7            & 6            & 5            & 8             \\
L-CNN                      & 17           & 11           & 8            & 25            \\
LETR                       & 8            & 8            & 8            & 8             \\
LSD                        & 111          & 112          & 61           & 139           \\
LSDNet                     & 13           & 13           & 13           & 13            \\
LSWMS                      & 20           & 25           & 20           & 19            \\
M-LSD                      & 98           & 103          & 99           & 111           \\
TP-LSD                     & 17           & 17           & 17           & 17            \\
ULSD                       & 27           & 26           & 25           & 28            \\
EDLines                    & \textbf{387} & \textbf{325} & \textbf{213} & \textbf{679}  \\
FLD                        & \uline{346}  & \uline{284}  & \uline{180}  & \uline{668}   \\
FSG                        & 39           & 38           & 21           & 51            \\
SOLD2                      & 3            & 3            & 4            & 7             \\
\hline
\end{tabular}
}
\end{table}

==> tables/pose_error_auc.tex <==
\begin{table}[!htb]
\centering
\caption{Pose error estimation: area under cumulative pose error}
\label{table:pose_error_auc}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{|l|l||lll|lll|lll|} 
\hline
\multirow{2}{*}{Detector}   & \multirow{2}{*}{Associator} & \multicolumn{3}{c|}{lr kt2}                      & \multicolumn{3}{c|}{of kt2}                      & \multicolumn{3}{c|}{fr3/cabinet}                 \\ 
\cline{3-11}
                            &                             & $AUC@1^\circ$  & $AUC@3^\circ$  & $AUC@5^\circ$  & $AUC@1^\circ$  & $AUC@3^\circ$  & $AUC@5^\circ$  & $AUC@1^\circ$ & $AUC@3^\circ$  & $AUC@5^\circ$   \\ 
\hline
\multirow{5}{*}{LSD}        & LBD                         & 15.19          & 27.87          & 33.28          & 15.98          & 31.29          & 36.80          & 1.50          & 8.27           & 13.28           \\
                            & DLD                         & 16.45          & 32.90          & 40.32          & 19.88          & 34.95          & 40.24          & 1.15          & 7.08           & 12.27           \\
                            & WLD                         & 13.16          & 26.89          & 33.37          & 9.63           & 20.47          & 24.85          & 0.89          & 7.03           & 11.98           \\
                            & LineTR                      & \textbf{29.45} & \textbf{54.41} & \textbf{62.69} & \textbf{33.60} & \textbf{59.31} & \textbf{66.98} & \uline{1.98}  & \uline{12.31}  & \uline{18.77}   \\
                            & SOLD2                       & 16.99          & 34.66          & 42.07          & \uline{22.26}  & 40.91          & 47.47          & \textbf{3.13} & \textbf{17.85} & \textbf{27.96}  \\ 
\cline{1-2}
\multirow{5}{*}{F-Clip@0.4} & LBD                         & 7.17           & 21.58          & 28.66          & 8.74           & 22.09          & 27.40          & 0.16          & 1.97           & 3.92            \\
                            & DLD                         & 10.21          & 28.37          & 35.92          & 7.17           & 19.97          & 26.11          & 0.31          & 2.02           & 3.61            \\
                            & WLD                         & 8.07           & 23.05          & 29.77          & 4.28           & 12.43          & 16.35          & 0.37          & 3.59           & 6.36            \\
                            & LineTR                      & 17.74          & 43.17          & \uline{53.56}  & 15.56          & \uline{42.24}  & \uline{52.03}  & 0.21          & 1.81           & 3.22            \\
                            & SOLD2                       & 14.66          & 37.50          & 46.17          & 11.08          & 28.89          & 37.22          & 0.65          & 5.57           & 11.13           \\ 
\cline{1-2}
\multirow{5}{*}{HAWP@0.7}   & LBD                         & 5.45           & 12.19          & 15.22          & 3.98           & 9.01           & 11.84          & 0.10          & 0.79           & 1.54            \\
                            & DLD                         & 6.53           & 15.69          & 19.43          & 2.11           & 6.84           & 10.24          & 0.10          & 0.59           & 1.18            \\
                            & WLD                         & 5.60           & 14.54          & 18.76          & 2.74           & 6.64           & 9.04           & 0.19          & 1.31           & 2.13            \\
                            & LineTR                      & 20.76          & \uline{43.44}  & 52.95          & 14.58          & 40.24          & 49.97          & 0.41          & 2.61           & 3.84            \\
                            & SOLD2                       & \uline{20.87}  & 43.33          & 50.82          & 13.99          & 29.92          & 37.47          & 0.89          & 7.49           & 12.46           \\
\hline
\end{tabular}
}
\end{table}
